Efficient Training for Visual Tracking with Deformable Transformer

Recent Transformer-based visual tracking models have showcased superior performance. Nevertheless, prior works have been resource-intensive, requiring prolonged GPU training hours and incurring high GFLOPs during inference due to inefficient training methods and convolution-based target heads. This intensive resource use renders them unsuitable for real-world applications. In this paper, we present DETRack, a streamlined end-to-end visual object tracking framework. Our framework utilizes an efficient encoder-decoder structure where the deformable transformer decoder acting as a target head, achieves higher sparsity than traditional convolution heads, resulting in decreased GFLOPs. For training, we introduce a novel one-to-many label assignment and an auxiliary denoising technique, significantly accelerating model's convergence. Comprehensive experiments affirm the effectiveness and efficiency of our proposed method. For instance, DETRack achieves 72.9% AO on challenging GOT-10k benchmarks using only 20% of the training epochs required by the baseline, and runs with lower GFLOPs than all the transformer-based trackers.

==> table/big_table.bk.tex <==

\definecolor{mygray}{gray}{0.93}
\begin{table*}[t]
    \footnotesize
    \centering
    \vspace{-2.5mm}
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc}
        \hline
        \rowcolor{mygray}
                                         &                                                     & \multicolumn{3}{c|}{GOT-10k* \cite{GOT-10k}}
                                         & \multicolumn{3}{c|}{TrackingNet \cite{TrackingNet}}
                                         & \multicolumn{3}{c|}{LaSOT \cite{LaSOT}}
                                         & \multicolumn{3}{c}{AVisT \cite{noman2022avist}}                                                                                                                                                                                                                                                                                                                                       \\
        \rowcolor{mygray}
        \multirow{-2}{*}{Tracker}
                                         & \multirow{-2}{*}{Source}
                                         & AO                                                  & SR$_{0.5}$                                   & SR$_{0.75}$
                                         & AUC                                                 & P$_{\text{Norm}}$                            & P
                                         & AUC                                                 & P$_{\text{Norm}}$                            & P
                                         & AUC                                                 & OP$50$                                       & OP$75$                                                                                                                                                                                                                                                                           \\
        \hline
        DETRack                          & Ours                                                & \textcolor{red}{72.9}                        & \textcolor{red}{82.1}  & \textcolor{red}{69.9}  & \textcolor{red}{83.2}  & \textcolor{red}{88.3}  & \textcolor{red}{83.1}  & \textcolor{red}{69.0}  & \textcolor{blue}{78.9} & \textcolor{red}{75.1}  & \textcolor{red}{54.5}  & \textcolor{red}{63.1}  & \textcolor{red}{45.2}  \\
        OSTrack \cite{ostrack}           & ECCV'22                                             & \textcolor{blue}{71.0}                       & \textcolor{blue}{80.4} & \textcolor{blue}{68.2} & \textcolor{blue}{83.1} & 87.8                   & 82.0                   & 69.1                   & 78.7                   & \textcolor{blue}{75.2} & -                      & -                      & -                      \\
        AiATrack \cite{aiatrack}         & ECCV'22                                             & 69.6                                         & 80.0                   & 63.2                   & 82.7                   & 87.8                   & 80.4                   & 69.0                   & \textcolor{red}{79.4}  & 73.8                   & -                      & -                      & -                      \\
        SimTrack \cite{simTrack}         & ECCV'22                                             & 68.6                                         & 78.9                   & 62.4                   & 82.3                   & 86.5                   & -                      & \textcolor{blue}{69.3} & 78.5                   & 74.0                   & -                      & -                      & -                      \\
        % RTS \cite{RTS}                & ECCV'22                                                       & -                                                 & -                      & -                      & 81.6                   & 86.0                   & 79.4                   & 69.7                   & 76.2                   & 73.7                   & 50.8                   & 55.7                   & 38.9                   \\
        Unicorn \cite{unicorn}           & ECCV'22                                             & -                                            & -                      & -                      & 83.0                   & 86.4                   & \textcolor{blue}{82.2} & 68.5                   & 76.6                   & 74.1                   & -                      & -                      & -                      \\
        MixFormer \cite{mixformer}       & CVPR'22                                             & 70.7                                         & 80.0                   & 67.8                   & \textcolor{blue}{83.1} & \textcolor{blue}{88.1} & 81.6                   & 69.2                   & 78.7                   & 74.7                   & \textcolor{blue}{53.7} & \textcolor{blue}{63.0} & \textcolor{blue}{43.0} \\
        ToMP \cite{TOMP}                 & CVPR'22                                             & -                                            & -                      & -                      & 81.2                   & 86.2                   & 78.6                   & 67.6                   & 78.0                   & 72.2                   & 51.6                   & 59.5                   & 38.9                   \\
        % SBT \cite{SBT}            & CVPR'22                                                       & 69.9                                              & 80.4                   & 63.6                   & -                      & -                      & -                      & 65.9                   & -                      & 70.0                   & -                      & -                      & -                      \\
        CSWinTT \cite{cswintt}           & CVPR'22                                             & 69.4                                         & 78.9                   & 65.4                   & 81.9                   & 86.7                   & 79.5                   & 66.2                   & 75.2                   & 70.9                   & -                      & -                      & -                      \\
        STARK \cite{STARK}               & ICCV'21                                             & 68.0                                         & 77.7                   & 62.3                   & 81.3                   & 86.1                   & 78.1                   & 66.4                   & 76.3                   & 71.2                   & 51.1                   & 59.2                   & 39.1                   \\
        KeepTrack \cite{KeepTrack}       & ICCV'21                                             & -                                            & -                      & -                      & -                      & -                      & -                      & 67.1                   & 77.2                   & 70.2                   & 49.4                   & 56.3                   & 37.8                   \\
        AutoMatch \cite{AutoMatch}       & ICCV'21                                             & 65.2                                         & 76.6                   & 54.3                   & 76.0                   & -                      & 72.6                   & 58.3                   & -                      & 59.9                   & -                      & -                      & -                      \\
        TransT \cite{transt}             & CVPR'21                                             & 67.1                                         & 76.8                   & 60.9                   & 81.4                   & 86.7                   & 80.3                   & 64.9                   & 73.8                   & 69.0                   & 49.0                   & 56.4                   & 37.2                   \\
        Alpha-Refine \cite{Alpha-Refine} & CVPR'21                                             & -                                            & -                      & -                      & 80.5                   & 85.6                   & 78.3                   & 65.3                   & 73.2                   & 68.0                   & 49.6                   & 55.7                   & 38.2                   \\
        TMT \cite{TMT}                   & CVPR'21                                             & 67.1                                         & 77.7                   & 58.3                   & 78.4                   & 83.3                   & 73.1                   & 63.9                   & -                      & 61.4                   & 48.1                   & 55.3                   & 33.8                   \\
        Ocean \cite{Ocean}               & ECCV'20                                             & 61.1                                         & 72.1                   & 47.3                   & -                      & -                      & -                      & 56.0                   & 65.1                   & 56.6                   & 38.9                   & 43.6                   & 20.5                   \\
        % PrDiMP \cite{prdimp} & CVPR'20                                                       & 63.4                                              & 73.8                   & 54.3                   & 75.8                   & 81.6                   & 70.4                   & 59.8                   & 68.8                   & 60.8                   & 43.3                   & 48.0                   & 28.7                   \\
        % SiamAttn \cite{siam}         & CVPR'20                                                       & -                                                 & -                      & -                      & 75.2                   & 81.7                   & -                      & 56.0                   & 64.8                   & -                      & -                      & -                      & -                      \\
        DiMP \cite{DiMP}                 & ICCV'19                                             & 61.1                                         & 71.7                   & 49.2                   & 74.0                   & 80.1                   & 68.7                   & 56.9                   & 65.0                   & 56.7                   & 41.9                   & 45.7                   & 26.0                   \\
        ATOM \cite{atom}                 & CVPR'19                                             & -                                            & -                      & -                      & 70.3                   & 77.1                   & 64.8                   & 51.5                   & 57.6                   & 50.5                   & 38.6                   & 41.5                   & 22.2                   \\
        SiamRPN++ \cite{SiamRPN++}       & CVPR'19                                             & 51.7                                         & 61.6                   & 32.5                   & 73.3                   & 80.0                   & 69.4                   & 49.6                   & 56.9                   & 49.1                   & 39.0                   & 43.5                   & 21.2                   \\
        \hline
    \end{tabular}
    \label{table-main}
    \caption{State-of-the-art comparison on GOT-10k, TrackingNet, LaSOT and AVisT. The best two results are shown in \textcolor{red}{red} and \textcolor{blue}{blue} fonts, respectively. We use * to denote that the results on GOT-10k are obtained following the official one-shot protocol.}
    \vspace{-2.5mm}
\end{table*}

